Sequential active learning of low-dimensional model representations for reliability analysis

To date, the analysis of high-dimensional, computationally expensive engineering models remains a difficult challenge in risk and reliability engineering. We use a combination of dimensionality reduction and surrogate modelling termed partial least squares-driven polynomial chaos expansion (PLS-PCE) to render such problems feasible. Standalone surrogate models typically perform poorly for reliability analysis. Therefore, in a previous work, we have used PLS-PCEs to reconstruct the intermediate densities of a sequential importance sampling approach to reliability analysis. Here, we extend this approach with an active learning procedure that allows for improved error control at each importance sampling level. To this end, we formulate an estimate of the combined estimation error for both the subspace identified in the dimension reduction step and surrogate model constructed therein. With this, it is possible to adapt the design of experiments so as to optimally learn the subspace representation and the surrogate model constructed therein. The approach is gradient-free and thus can be directly applied to black box-type models. We demonstrate the performance of this approach with a series of low- (2 dimensions) to high- (869 dimensions) dimensional example problems featuring a number of well-known caveats for reliability methods besides high dimensions and expensive computational models: strongly nonlinear limit-state functions, multiple relevant failure regions and small probabilities of failure.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage[margin=2.5cm]{geometry}% by courtesy of Mico
\usepackage{subfig} % was: subfignarms.sty
\usepackage{bm}
\usepackage{bbm}
\usepackage{amsmath}
\usepackage{multirow}
\usepackage{pdflscape}
\usepackage{mathtools}
\usepackage{tabularx}
\usepackage{overpic}
\usepackage{placeins}
\usepackage{caption}
\usepackage{amssymb}
\usepackage{cleveref}
\usepackage{lineno}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{etoolbox}
\usepackage{tikz}
\usetikzlibrary{arrows.meta}
\tikzset{%
	>={Latex[width=2mm,length=2mm]},
	% Specifications for style of nodes:
	base/.style = {rectangle, rounded corners, draw=black,
		minimum width=2cm, minimum height=1.25cm,
		text centered,font=\rmfamily\footnotesize},
	output/.style = {base, fill=black!15},
	input/.style = {base, fill=green!15},
	truth/.style = {base, fill=black!35},
	process/.style = {base, fill=white}
}

\crefname{equation}{Eq.}{Eqs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{tabular}{Tab.}{Tabs.}
\crefname{section}{Section}{Sections}
\crefname{subsection}{Subsection}{Subsections}
\crefname{algorithm}{Algorithm}{Algorithms}

\makeatletter
% start with some helper code
% This is the vertical rule that is inserted
\newcommand*{\algrule}[1][\algorithmicindent]{%
	\makebox[#1][l]{%
		\hspace*{.2em}% <------------- This is where the rule starts from
		\vrule height .75\baselineskip depth .25\baselineskip
	}
}

\newcount\ALG@printindent@tempcnta
\def\ALG@printindent{%
	\ifnum \theALG@nested>0% is there anything to print
	\ifx\ALG@text\ALG@x@notext% is this an end group without any text?
	% do nothing
	\else
	\unskip
	% draw a rule for each indent level
	\ALG@printindent@tempcnta=1
	\loop
	\algrule[\csname ALG@ind@\the\ALG@printindent@tempcnta\endcsname]%
	\advance \ALG@printindent@tempcnta 1
	\ifnum \ALG@printindent@tempcnta<\numexpr\theALG@nested+1\relax
	\repeat
	\fi
	\fi
}
% the following line injects our new indent handling code in place of the default spacing
\patchcmd{\ALG@doentity}{\noindent\hskip\ALG@tlm}{\ALG@printindent}{}{\errmessage{failed to patch}}
\patchcmd{\ALG@doentity}{\item[]\nointerlineskip}{}{}{} % no spurious vertical space
% end vertical rule patch for algorithmicx
\makeatother

\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\heading}[1]{\multicolumn{1}{c}{#1}}

% increase vertical spacing in table rows
\renewcommand{\arraystretch}{1.5}

\makeatletter
% Reinsert missing \algbackskip
\def\algbackskip{\hskip-\ALG@thistlm}
\makeatother

\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

% Sets running headers as well as PDF title and authors
\headers{Sequential active learning of low-dimensional model representations for RA}{M. Ehre, I. Papaioannou, B. Sudret and D. Straub}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{Sequential active learning of low-dimensional model representations for reliability analysis\thanks{Submitted to the editors DATE.
\funding{This project was supported by the German Research Foundation (DFG) through Grant STR 1140/6-1 under SPP 1886.}}}

% Authors: full names plus addresses.
\author{Max Ehre\thanks{Engineering Risk Analysis Group, Technical University of Munich
  (\email{max.ehre@tum.de},\email{iason.papaioannou@tum.de},\email{straub@tum.de}).}
\and Iason Papaioannou\footnotemark[2]
\and Bruno Sudret\thanks{Chair of Risk, Safety and Uncertainty Quantification, ETH Z{\"u}rich
  (\email{sudret@ibk.eth.ch}).}
\and Daniel Straub\footnotemark[2]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

